Faithiful Embeddings for EL++ Knowledge Bases

Recently, increasing efforts are put into learning continual representations for symbolic knowledge bases (KBs). However, these approaches either only embed the data-level knowledge (ABox) or suffer from inherent limitations when dealing with concept-level knowledge (TBox), i.e., they cannot faithfully model the logical structure present in the KBs. We present BoxEL, a geometric KB embedding approach that allows for better capturing the logical structure (i.e., ABox and TBox axioms) in the description logic EL++. BoxEL models concepts in a KB as axis-parallel boxes that are suitable for modeling concept intersection, entities as points inside boxes, and relations between concepts/entities as affine transformations. We show theoretical guarantees (soundness) of BoxEL for preserving logical structure. Namely, the learned model of BoxEL embedding with loss 0 is a (logical) model of the KB. Experimental results on (plausible) subsumption reasonings and a real-world application for protein-protein prediction show that BoxEL outperforms traditional knowledge graph embedding methods as well as state-of-the-art EL++ embedding approaches.

==> 1_introduction.tex <==
\section{Introduction}

\todo{maybe think more and talk more about interleaving classical and our method
1. apply classical method to answer query. If it cannot provide yes/no answer, employ our method.
2. When applying our method, try to combine it with classical method to
inferences that are inconsistent with the TBox}

\hspace*{\fill} \textit{Spatial thinking is the foundation of abstract thought.} \\
\hspace*{\fill} —\textit{Barbara Tversky (2019) p. 72, p. 142}

The Sixth Law of Cognition--spatial thinking tells us that human reasoning can be interpreted as spatial (geometric) operations over abstract concepts. This cognitive intuition motivates the development of AI to represent concepts with geometric objects, which is given through the \textit{geometric representation learning}. We consider the problem of geometric representation for symbolic knowledge bases (KBs), such that the logical structure in the KB is explicitly preserved in the embedding space for logic reasoning. 

One of the standard ways to express logical structure in KBs is via ontologies, which provides a \textit{conceptualization} of objects and their relationships constraining viable logical interpretations. Model-theoretic languages such as Description Logic (DL) are a family of languages allowing for expressing ontology-based KBs through logical statements (a.k.a axioms). 
These logical statements are divided into three parts: 1) ABox is a set of logical statements constraining individuals e.g. $\rel{isFatherOf}(\inst{John}, \inst{Peter})$; 2) TBox is a set of logical statements constraining concepts e.g. $\concept{Parent} \sqsubseteq \concept{Person}$.
% Note that in other materials, TBox together with an RBox are called an \emph{ontology} while the combination of an ontology and ABox is called the Knowledge Graphs (KG). 
 
 \begin{figure}
    \centering
    \includegraphics[width=\linewidth]{imgs/counter_example.pdf}
    \caption{Two counterexamples of BallEL that BoxEL can address. (a) Ball embedding cannot express concept equivalence $\concept{Parent} \sqcap \concept{Male} \equiv \concept{Father}$ with intersection. (b) The \textit{translation} of BallEL cannot model relation (e.g. $\rel{isChildOf}$) between $\concept{Person}$ and $\concept{Parent}$ when they have different sizes. These two issues can be solved by \textit{Box} embedding and modelling relation as \textit{affine transformation}, respectively.}
    \label{fig:example_intersection}
    \vspace{-0.1cm}
\end{figure}


Recently, geometric representation methods have been explored on embedding KBs expressed in model-theoretic DL languages like Extended Existential Language ($\mathcal{EL}^{++}$) \cite{kulmanov2019embeddings} that supports conjunction and full existential quantification and \textit{Attributive Language with Complements} ($\mathcal{ALC}$) \cite{ozccep2020cone} that further supports logical negation. 
% Although $\mathcal{ALC}$ is more expressive, 
We focus on $\mathcal{EL}^{++}$, which is the underlying formalism for the standardized Web Ontology Language (OWL2 EL) \cite{graua2008web}, as it is computationally tractable and has multiple applications in biomedical ontologies \cite{gene2015gene, rector1996galen}. 
For $\mathcal{EL}^{++}$ embeddings, the most relevant work is BallEL \citep{kulmanov2019embeddings} that represents concepts as open $n$-balls and relations as \textit{translations} among $n$-balls analogous to the translations in TransE \citep{BordesUGWY13}. BallEL has been shown to have advantages over classical KGEs on protein-protein interactions.  BallEL$^{++}$~\cite{mondala2021emel} recently extends BallEL to support RBox embeddings and shows some performance gains on subsumption reasoning over biomedical ontologies. However, BallEL and BallEL$^{++}$ suffer from several major issues. 
\begin{itemize}
    \item Balls are not closed under intersection, which limits the extent to which some simple and common logic structures can be captured. For example, Fig.~\ref{fig:example_intersection}(a) illustrates that it is impossible to capture $\concept{Parent} \sqcap \concept{Male} \equiv \concept{Father}$ with balls because the intersection $\concept{Parent} \sqcap \concept{Male}$ that is supposed to represent $\concept{Father}$, is not a ball.
    \item It is well known that the simple \textit{translation} as used in TransE suffers from various limitations~\citep{wang2014knowledge}. In the context of concept embeddings, new problems occur.
    % For example, Fig. \ref{fig:example_intersection}(b) shows that given $\concept{Parent} \sqsubseteq \concept{Person}$, it is impossible to \textit{translate} the larger concept $\concept{Person}$ into the smaller one $\concept{Parent}$ preserves the structure of $\exists \rel{isChildOf}.\concept{Person} \sqsubseteq \concept{Parent}$,
    % \footnote{Under the \textit{translation} setting, the embeddings will simply become $\concept{Parent} \equiv \concept{Person}$, which is obviously not we want as we can express $\concept{Parent} \not\equiv \concept{Person}$ with $\mathcal{EL}^{++}$ by adding additional propositions like $\concept{Children} \sqcap \concept{Parent} \sqsubseteq \bot$ and $\concept{Children} \sqsubseteq \concept{Person}$} as it is not allowed to scale the size with translation.
    For example, Fig. \ref{fig:example_intersection}(b) illustrates the embeddings for concepts and relation in the axiom  $\exists \rel{isChildOf}.\concept{Person} \sqsubseteq \concept{Parent}$ assuming the existence of another axiom $\concept{Parent} \sqsubseteq \concept{Person}$. In this case it is impossible to \textit{translate} the larger concept $\concept{Person}$ into the smaller one $\concept{Parent}$,\footnote{Under the \textit{translation} setting, the embeddings will simply become $\concept{Parent} \equiv \concept{Person}$, which is obviously not what we want as we can express $\concept{Parent} \not\equiv \concept{Person}$ with $\mathcal{EL}^{++}$ by adding additional propositions like $\concept{Children} \sqcap \concept{Parent} \sqsubseteq \bot$, $\concept{Children} \sqsubseteq \concept{Person}$ and $\concept{Children}(a)$} as it does not allow for scaling the size.
    \item BallEL and BallEL$^{++}$ consider concept assertions and role assertions as special cases of concept inclusions. While this is empirically valid, this simple treatment does not distinguish entities and concepts (i.e. they encode entities as regular balls), losing some theoretical guarantee that we will discuss later.
    % encodes entities and concepts, but instead, it transforms concept assertions and role assertions into. This simple method limits the distinguish of concepts and entities. Intuitively, a concept can contain an infinite number of entities while an entity should have minimum volume.  
    % this case can be trivially expressed $\concept Parent \not\equiv \concept Person$ with DL $\mathcal{EL}^{++}$ by adding additional propositions like $\concept Children \sqcap \concept Parent \sqsubseteq \bot$ and $\concept Children \sqsubseteq \concept Person$, as well as the non-emptiness restrictions by $\{a\} \sqsubseteq Children$ and $\{b\} \sqsubseteq Parent$ }, 
    % The simple \textit{translation} vector cannot capture \textit{role inclusion} and \textit{role chain}. For example, $hasChild \sqsubseteq isAncestorOf$ simply means that they should be the same vector. This problem limits the expressivity of embeddings of logical RBox statements.
\end{itemize}
% Specifically, 
% Our aim is to learn a KB embedding that incorporates the DL $\mathcal{EL}^{++}$ such that the logical statements in the ABox and TBox become isomorphic to a lattice structure over a set of subspaces of the vector space.
% EL embedding that incorporates the $\mathcal{EL}^{++}$ operators (conjunction, existential quantification) and can express the bottom concept $\bot$. 
% DL $\mathcal{EL}^{++}$ that arrows for concept conjunction and full existential restriction. 
% Our aim is to learn a logic-preserved KB embedding that incorporates the $\mathcal{EL}^{++}$ operators (conjunction, existential quantification) and can express the bottom concept $\bot$. 
% Geometric embedding models, in which the objects are embedded with geometric objects (i.e. disks, cones and boxes), have shown promising results on representations of symbolic data like words, entities, concepts and queries. 
% Probabilistic Box Embedding is one of the well-defined techniques, possessing the advantages of modeling complex probabilistic distributions. 
% Knowledge graph embeddings (KGEs) \citep{bordes2013translating, wang2014knowledge} map entities and relations into a low-dimensional space (typically $R^n$) and have been applied to a variety of downstream tasks like link prediction, question answering and knowledge alignment. Traditional KGE methods concentrate mainly on exploiting the instance-level data (ABox) but do not consider the constraints and characteristics of the underlying schema or ontology (TBox). Recently, ...
% Ontology embeddings, which exploit TBox data to map classes, relations, and instances in the ontologies into a vector space, can preserve certain syntactic properties of the ontology axioms and their deductive closure. 

To overcome these limitations, we consider modeling concepts in the KB as \textit{boxes} (i.e. axis-aligned hyperrectangles), encoding entities as points inside the boxes that they should belong to, and the relations as the \textit{affine transformation} between boxes and/or points. Fig.~\ref{fig:example_intersection}(a) shows that a Box embedding with closed form of intersection and the \textit{affine transformation} (Fig.~\ref{fig:example_intersection}(b)) can naturally capture the cases that are not possible in Ball embeddings. 
%struggle with. 
In this way, we present BoxEL$^{++}$ for embedding  %ontology-based 
KBs expressed by DL $\mathcal{EL}^{++}$, in which the interpretation functions of an $\mathcal{EL}^{++}$ theory in the KB can therefore be represented by the geometric transformations between boxes/points. 
We show that BoxEL$^{++}$ overcomes inherent limitations of existing approaches and provides some analytical guarantees (a.k.a. \textit{soundness}).
We formulate BoxEL$^{++}$ as an optimization task by designing and minimizing various loss terms defined for each logical statement in the KB.
%ontologies. 
\par
To summarize, our contributions are as follows:
\begin{itemize}
    \item We present BoxEL$^{++}$, a Box embedding method for modeling logical structure expressed by the DL language $\mathcal{EL}^{++}$.
    %in the ontologies. 
    % \item We provide theoretical analysis with regard to the 
    % guarantees for preserving logic implications of symbolic KBs expressed by $\mathcal{EL}^{++}$ theories. 
    \item We show theoretical guarantees (\textit{soundness}) of BoxEL$^{++}$ for preserving logic structure in the KB. Namely, BoxEL$^{++}$ finds an interpretation function that satisfies all axioms in the KB.
    \item We demonstrate the superiority of BoxEL$^{++}$ on the subsumption reasoning task for various biomedical ontologies and predicting protein-protein interactions in a biomedical knowledge graph. The code is available for reproducibility.\footnote{https://github.com/Box-EL/BoxEL}%footnote should be after the period.
\end{itemize}
